Language Features Matter: Effective Language Representations for Vision-Language Tasks

Shouldn't language and vision features be treated equally in vision-language (VL) tasks? Many VL approaches treat the language component as an afterthought, using simple language models that are either built upon fixed word embeddings trained on text-only data or are learned from scratch. We believe that language features deserve more attention, and conduct experiments which compare different word embeddings, language models, and embedding augmentation steps on five common VL tasks: image-sentence retrieval, image captioning, visual question answering, phrase grounding, and text-to-clip retrieval. Our experiments provide some striking results; an average embedding language model outperforms an LSTM on retrieval-style tasks; state-of-the-art representations such as BERT perform relatively poorly on vision-language tasks. From this comprehensive set of experiments we propose a set of best practices for incorporating the language component of VL tasks. To further elevate language features, we also show that knowledge in vision-language problems can be transferred across tasks to gain performance with multi-task training. This multi-task training is applied to a new Graph Oriented Vision-Language Embedding (GrOVLE), which we adapt from Word2Vec using WordNet and an original visual-language graph built from Visual Genome, providing a ready-to-use vision-language embedding: http://ai.bu.edu/grovle.

==> multitask.tex <==
\subsection{Multi-Task Training}
\label{sec:specalized}

A drawback of using pretrained word embeddings like Word2Vec or the retrofitting process from Section~\ref{subsec:retrodetails} is that they are trained solely on text data.  While our Visual Genome Graph provides some information on how words in our vocabulary are used for visual data, it doesn't provide any sense of the visual similarity between different words or any nuances that may be necessary to perform a particular vision-language task.  To address this, we fine-tune our word embeddings across five common vision-language tasks. We additionally perform this multi-task training to see if there are trends found in the transferability amongst retrieval and generation problems, in order to increase performance in future work. %: image-sentence retrieval, phrase grounding, text-to-clip retrieval, image captioning, and visual question answering.

We start by performing a single pretraining of the embedding, i.e. we train an embedding during one task for use in another. This will reveal if vision-language tasks can generalize and boost performance by tuning the embedding to contain useful visual information. In the single pretrain experiments, fine tuning is allowed in both tasks. Lastly, we provide results for a four task and five task multi-trained embedding. The four task experiments are performed with the final task embedding fixed, and the five task allows for fine-tuning during the last task.

For each dataset/task in the four and five task experiments, we keep the $K$ most informative features frozen when training any subsequent task, which enables us to diminish the effect of catastrophic forgetting when fine-tuning on a new task. For an embedding of size $D$ and $T$ tasks, $K=\frac{D}{T}$, \ie $K = 60$ in our experiments. We evenly split the $K$ features for tasks with multiple datasets.  Features that were tuned on a task are ranked according to variance and frozen before training on the next dataset/task.  The end result is a pretrained word embedding which can simply be ``dropped in'' to existing models to improve performance across many vision-language tasks.

==> retrofitting.tex <==
 \section{Learning Word Embeddings for Vision-Language Tasks}
 To train a word embedding for vision-language tasks, we begin by retrofitting Word2Vec with lexical databases which contain semantic relationships between words which we shall discuss in Section~\ref{subsec:retrodetails}.  We describe the semantic relationships used to modify our word embeddings in Section~\ref{subsec:graph}.  Finally, we fine-tune the embeddings on five common vision-language tasks using the procedure outlined in Section~\ref{sec:specalized}.
 
 %We begin to learn our vision-language representations by retrofitting the Word2Vec embeddings by taking advantage of lexicons which provide relational information not easily learned using word context in large language corpora. 
 %Section~\ref{subsec:retrodetails} reviews the belief propagation approach proposed by~\citet{FaruquiNAACL} to modify the word embeddings using information obtained from a word relationship graph. Section~\ref{subsec:wordnet} describes the word relationship graph built on WordNet~\cite{wordnet} used by~\citet{FaruquiNAACL}.  In Section~\ref{subsec:visgenome} we discuss our proposed word relationship graph built from a large vision-language corpus extracted from the Visual Genome dataset~\cite{krishnavisualgenome}, which provides a sense of the differences in how words are used when describing visual data.  After retrofitting our embeddings, we perform an iterative multi-task training procedure which we discuss in Section~\ref{sec:specalized} to learn a single embedding which generalizes well across many vision-language tasks.

\label{sec:retro}
\subsection{Retrofitting Word Embeddings}
\label{subsec:retrodetails}
In this section we review the approach of Faruqui~\etal\cite{FaruquiNAACL}, who proposed a graph based learning technique which retrofits additional semantic knowledge onto pretrained word embeddings. This approach is used as a post-processing step for a pretrained embedding, and is compared experimentally with other post-processed embeddings such as Visual Word2Vec and Fisher Vectors. Given a vocabulary $V$ with words $\{w_1, w_2, ..., w_n\}$ and its corresponding word embedding $\hat{Q}$, where $\hat{q}_i$ is the embedding for $w_i$, belief propagation is performed to obtain a new embedding $Q$ which minimizes the distances between the embedding representing each word and its neighbors. These neighbors are defined as edges $E$ between words in a graph.  $L2$ regularization is performed between the original and new word embeddings to help prevent overfitting, \ie,

\begin{equation}
    L_{reg}(Q, \hat{Q}) = \sum_{i=1}^{n} \alpha_i\|q_i-\hat{q}_i\|^2,
    \label{eq:l2_reg}
\end{equation}

\noindent where $\alpha_i$ is a weight controlling the strength of the regularization. As done in Faruqui~\etal\cite{FaruquiNAACL}, we set $\alpha_i$ to be equal to the number of neighbors of $w_i$. We find that this $L2$ regularization is necessary whenever we are updating the word embeddings (\ie we also use it during multi-task training described in Section~\ref{sec:specalized}). The final training objective to perform the retrofitting is then,

\begin{equation}
    \Psi_{retro}(Q, \hat{Q}) = L_{reg} + \sum_{(i,j) \in E} \beta_{ij}\|q_i-q_j\|^2, 
    \label{eq:retrofit}
\end{equation}

\noindent $\beta$ is the weight controlling the importance the distance to the neighbors has on the final embedding. We set $\beta=1$ and solve the system of linear equations defined by Eq.~(\ref{eq:retrofit}) using an efficient iterative updating method~\cite{itermethod} for 10 iterations using the implementation provided by Faruqui~\etal\cite{FaruquiNAACL}. Although Faruqui~\etal\cite{FaruquiNAACL} constructed lexicons using WordNet~\cite{wordnet}, FrameNet~\cite{framenet}, and the Paraphrase Database~\cite{ppdb} we used only the WordNet graph, which we shall now describe, since it contains the largest vocabulary with the most edges. 
%\par The authors have shown significant improvement using this technique as a post-processing step compared to others~\cite{YuDredzeAACL} which alter the embeddings during the learning process.  Retrofitting is also advantageous as it is more generalizable; it can be performed on any word embedding regardless of the vector training model.

\subsection{Word Relation Graph Construction}
\label{subsec:graph}
Below we describe the two methods we use to create the edges between words which share some semantic relation. We use these edges to retrofit the word embeddings with the process described in Section~\ref{subsec:retrodetails}.  These retrofitted word embeddings are what we use as input into a multi-task training procedure to fine-tune the word embeddings for five common vision-language tasks which we will describe in Section~\ref{sec:specalized}.
\smallskip

\noindent\textbf{WordNet Graph.}  WordNet~\cite{wordnet} is a hierarchical lexical database which organizes nouns, adjectives, verbs and adverbs into sets of synonyms, called \textit{synsets}, and defines semantic relations to associate them. Following Faruqui~\etal\cite{FaruquiNAACL}, we construct a graph by creating links between words if there is synonym, hypernym, or hyponym relationship in WordNet between them.
\smallskip

\noindent\textbf{Visual Genome Graph.} 
\label{subsec:visgenome}
Visual Genome~\cite{krishnavisualgenome} contains a wealth of language annotations for 108K images, which include descriptions of entities in an image, their attributes, relationships between multiple entities, and both whole image and region-based question answer (QA) pairs. Each instance in these annotations is considered a single sample which we tokenize and remove stopwords from. We compute co-occurrence statistics over pairs of words within the sample and remove pairs that occur less than 50 times, resulting in 322,928 pairs for 12,849 words. For each word we compute a pointwise mutual information (PMI) score for all pairs it occurs in, and create links between the top ten words. This results in a graph where words that occur frequently together when describing visual data are linked together.

%The Visual Genome Graph is constructed from a corpus of phrases and sentences extracted from the Visual Genome Dataset~\cite{krishna2017dense}.  The dataset comprises of seven components, of which the following four are used to construct the lexicon: relationships, attributes, region descriptions and question answer (QA) pairs.  The region descriptions component contains a collection of descriptions based on different regions of each image.  The attributes and relationships associated with each object collected from region descriptions make up the attributes and relationships components respectively.  In the QA component, each image contains freeform and region-based QAs where the former is based on the entire image and the latter on selected regions. 

%Similar to the preprocessing done in the training of the skip-gram text model, we tokenized each phrase parsed from the above-mentioned components and removed stop words.  This was done to avoid frequent co-occurrences of word pairs since the retrofitting of the embeddings do not benefit much from word pairs that include extremely common words such as 'the' and 'in'.  Then, based on the idea of bigram counts, we computed the co-occurrence statistics for each word pair that occurs together in a phrase.  For simplicity, we did not account for the ordering of words within each pair by sorting them in lexicographical order.  We further refined these statistics by removing all word pairs that occur less than a selected threshold.  In our case, we used the threshold 50.    

%These co-occurrence statistics are used to compute the pointwise mutual information (PMI) value for each word pair.  Let ${(w_1, w_2)}$ denote each lexicographically sorted word pair.  To create the lexicon, for each word $w_1$, we selected the bigrams, starting with $w_1$, with the top ten PMI values.   The ontology constructed from this lexicon explicitly incorporates visual concepts into the embeddings by relating words that occur together frequently in image annotations and visual descriptions.

==> supp_material.tex <==
\subsection{Datasets}
\label{subsec:datasets}

\noindent\textbf{Flickr 30K~\cite{young2014image}.}  This dataset consists of 32K images obtained from the Flickr website, each of which has been annotated with five descriptive captions. We use the splits of Plummer~\etal~\cite{flickrentitiesijcv}, which separate the dataset into 30K/1K/1K train/test/validation images which we use for the image-sentence retrieval and phrase grounding tasks.
\smallskip

\noindent\textbf{MSCOCO~\cite{lin2014microsoft}.}  This dataset links 123K images for the training and validation sets (80K/40K images, respectively), each of which is annotated with five descriptive captions.  For the image-sentence retrieval experiments, we use the test/validation splits from Wang~\etal~\cite{wangTwoBranch2017}, which consists of 1K images for each split, for a total of 2K images, randomly sampled from the validation set. For image captioning experiments, use the splits from Chen~\etal~\cite{tencent}, which reserves 5k images each for validation and testing.
\smallskip

\noindent\textbf{Flickr30K Entities~\cite{flickrentitiesijcv}.}  This dataset augments the Flickr30K dataset with 276K bounding boxes which are linked to noun phrases in the descriptive captions.  We use the same splits as the Flickr30K dataset, resulting in 14.5K instances across the 1K images in the test set for the phrase grounding task.  Following~\cite{flickrentitiesijcv,rohrbach2015,wangTwoBranch2017}, we use the union of the bounding boxes for the ground truth box of a phrase which is linked to multiple boxes.
\smallskip

\noindent\textbf{ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014}.}  This dataset augments the 20K images from the IAPR RC-12 dataset~\cite{Grubinger06theiapr} with 120K region descriptions. We split the splits of Hu~\etal~\cite{hu2016natural}, which split the images evenly into train/validation and test sets (10K each), resulting in about 60K instances in each split. 
\smallskip

\noindent\textbf{DiDeMo~\cite{hendricks17iccv}.}  This dataset consists of just over 10,000 videos, each of which has between 3-5 video segment descriptions.  We use the splits provided by Hendricks~\etal~\cite{hendricks17iccv}, which splits the videos into sets of 8.4K/1K/1K for train/test/validation.
\smallskip

\noindent\textbf{VQA v2~\cite{balanced_vqa_v2}.}   This dataset augments images from MSCOCO with QA pairs.  The training, validation and test image sets contain 83K, 41K, and 81K images, respectively.  This constitutes 444K, 214K, and 448K questions for training/validation/testing splits.  Each training and validation question has ten answers provided.

\subsection{Task Methods}
\label{subsec:task_methods}

\noindent\textbf{Image-Sentence Retrieval.}  We use the implementation of the Embedding Network~\cite{wangTwoBranch2017} provided by the authors in our experiments.  This model uses two branches, one for text and one for images, to learn a projection to a shared embedding space where Euclidean distance is used to measure similarity between images and sentences.  We use the default parameters and data processing in the author's implementation, except that we compute the visual representation for each image  using a 152-layer ResNet~\cite{He2015} which has been trained on ImageNet~\cite{imagenet_cvpr09}.  Additionally, we use 448x448 crops rather than the 224x224 pixel crops used by Wang~\etal~\cite{wangTwoBranch2017} as done in prior work, \eg~\cite{Zhang_2018_ECCV,Nam_2017_CVPR}.  Following~\cite{wangTwoBranch2017,Zhang_2018_ECCV,Nam_2017_CVPR}, we keep the CNN parameters fixed for a fair comparison.  By default this model uses an Average Embedding language model.  When we use the LSTM language model, we use a hidden state of 512-D.  We set $\alpha$ in Eq.~(\ref{eq:l2_reg}) to be 1e-4 when fine-tuning the Average Embedding model and 1e-6 for the LSTM model.
\smallskip

\noindent\textbf{Phrase Grounding.} To evaluate our word embeddings on this task, we use implementation of CITE network~\cite{plummerCITE2017} used in Plummer~\etal~\cite{plummerArxiv2018}.  This model learns a set of embeddings which share some parameters, each of which captures a different concept important for phrase grounding.  We use the parameters and feature representation learned from fine-tuning a 101-layer ResNet and Region Proposal Network for the grounding task used in Plummer~\etal~\cite{plummerArxiv2018}.  This model also uses an Average Embedding language model by default, and we use 256-D hidden state for our LSTM experiments.  We set $\alpha$ in Eq.~(\ref{eq:l2_reg}) to be 1e-5 for both datasets.
\smallskip

\noindent\textbf{Text-to-clip.} As of this writing, none of the methods on the DiDeMo dataset which outperform the baseline model of Hendricks~\etal\cite{hendricks17iccv} have publicly available code for the text-to-clip task (\eg~\cite{chenEMNLP2018,Liu_2018_ECCV}).  As a result, we used the CITE network for the text-to-clip task since it performed better than the baseline model as well as better than the phrase-region grounding Similarity Network~\cite{wangTwoBranch2017} and straightforward adaptations of the R-C3D model~\cite{Xu2017iccv} in our experiments.  We learn $K=8$ concept embeddings for this dataset and use the VGG~\cite{simonyan2014very} features for the visual representation provided by Hendricks~\etal\cite{hendricks17iccv}.  We use a 512-D hidden state for our LSTM models, and set $\alpha$ in Eq.~(\ref{eq:l2_reg}) to 0.05.  This dataset likely required additional regularization when fine-tuning its embeddings due to its relatively small size.
\smallskip

\noindent\textbf{Image Captioning.}
We use a PyTorch implementation
%We use a PyTorch implementation 
\footnote{https://github.com/chenxinpeng/ARNet/tree/4431270e9e74ec55ab3abc0bb3c9b1ebce671c4a/image_captioning}
of the ArNet architecture provided by the authors of~\cite{tencent}. This model builds off of the original Neural Image Captioning (NIC) architecture of~\cite{vinyalsCVPR2015} by adding an additional LSTM to reconstruct previous hidden states. NIC follows an encoder-decoder paradigm inspired by machine translation, in which the probability of a sentence given an image is maximized. A CNN encodes an image which is then fed into a decoder LSTM to form a natural language sentence. We set the regularization coefficient of the NIC loss, $alpha$, to be $5e-2$ when fine-tuning the word embeddings. ArNet's additional stacked LSTM takes a current hidden state as input and tries to generate the previous hidden state as output. This can be viewed as a "soft" zoneout strategy as the model adaptively learns how to reconstruct the last hidden state at each time step, as opposed to the typical zoneout regularizer which makes a binary choice between previous and current hidden states.
%of the Neural Image Captioning (NIC) model~\cite{vinyalsCVPR2015} for this task. This model follows an encoder-decoder paradigm inspired by machine translation, in which the probability of a sentence given an image is maximized. A CNN encodes an image which is then fed into a decoder LSTM to form a natural language sentence. Unlike the results reported in Vinyals~\etal~\cite{vinyalsCVPR2015}, we use a single model rather than an ensemble, and use a 152-layer ResNet pretrained on ImageNet as our image encoder. We set $\alpha=5e-2$ in Eq.~(\ref{eq:l2_reg}) when fine-tuning the word embeddings.
%The base model published learned embeddings from scratch of dimension $256$, and the rest of our experiments report results for embedding dimension $300$, as they are based on Word2Vec. The only exception to this includes the HGLMM embedding experiments which are of dimension $6000$ as they are based on fisher vectors. We also present compressed $300$-dimensional HGLMM features for better comparison, and heightened motivation for the use of our enhanced embeddings. The authors publish their best results obtained with the use of ensemble methods and dropout regularization. We incorporate a dropout rate of $p=0.2$ in the LSTM layer, but the location and rate of dropout used for the NIC results was not provided in the previous work. We reproduce the baseline results (with embedding dimension $256$) for proper comparison for these reasons.
\smallskip

\noindent\textbf{Visual Question Answering.}
We use the authors' implementation of the End-to-End Module Networks~\cite{hu2017learning} as our VQA model. This network learns to decompose natural language questions into sub-tasks and assembles question-specific deep networks from neural modules to solve its corresponding sub-task.  %It also learns the network parameters simultaneously.  
There are two parts to the training process of this model: cloning expert and policy search. Since the policy search improves the model by only 0.7\% while adding significant training time, we report results only using the cloning expert.  We use the default parameters in the implementation and follow the authors' data pre-processing steps. When we include L2 regularization on the word embeddings, we set its weight to be 5e-4. Note that we report results using the VQA v2 dataset, whereas  Hu~\etal~\cite{hu2017learning} reported results on VQA v1.

Preliminary experiments showed GloVe performed similarly to Word2Vec (some provided below), Thus, we didn't include it due to space constraints.
\begin{table}[htb!]
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|rl|c|c|c|c|}
\hline
& Task & \multicolumn{2}{|c|}{Image-Sentence Retrieval} & \multicolumn{2}{|c|}{Phrase Grounding}\\
%\hline
%& Dataset & [48] & [28] & [37] & [19]\\
\hline
& Model & \multicolumn{2}{|c|}{[44]} & \multicolumn{2}{|c|}{[35]}\\
\hline
& Word2Vec & 71.9 & 79.9 & 69.43 & 51.70\\
& GloVe & 71.9 & 80.3 & 68.43 &  51.83\\
\hline
\end{tabular}
%\caption{Comparison of Word2Vec and Glove.}
\vspace{-3mm}
\end{table}
